A Gradient Estimator for Time-Varying Electrical Networks with Non-Linear Dissipation

We propose a method for extending the technique of equilibrium propagation for estimating gradients in fixed-point neural networks to the more general setting of directed, time-varying neural networks by modeling them as electrical circuits. We use electrical circuit theory to construct a Lagrangian capable of describing deep, directed neural networks modeled using nonlinear capacitors and inductors, linear resistors and sources, and a special class of nonlinear dissipative elements called fractional memristors. We then derive an estimator for the gradient of the physical parameters of the network, such as synapse conductances, with respect to an arbitrary loss function. This estimator is entirely local, in that it only depends on information locally available to each synapse. We conclude by suggesting methods for extending these results to networks of biologically plausible neurons, e.g. Hodgkin-Huxley neurons.

==> draft.tex <==
Since $\dot{q}(t) = i(t)$, we have:

\begin{equation}\label{fracmem}
    \frac{df}{dq} \tensor{_t}{D}{^{1/2}_{b}} \frac{\partial \mathcal{L}}{\partial \left(\tensor{^C_a}{D}{^{1/2}_{t}}f \right)} = \left(\frac{df}{dq}\right)^{2} i(t)
\end{equation}

We can now compare the Euler-Lagrange term obtained via the fractional action to the memristor Euler-Lagrange term obtained in \cite{shragowitz1988set}, which is derived with the use of a Rayleigh dissipation function rather than the variation of an action:

\begin{equation}\label{rayleighmem}
    \frac{d}{dt} \frac{\partial R_{a}}{\partial q} =  \frac{d\Phi(q)}{dt} = \frac{d\Phi}{dq} \frac{dq}{dt} = M(q) i(t)
\end{equation}

Here, $R_{a}$ is a Rayleigh dissipation function, $\Phi(q)$ is the charge-flux constitutive relation of the memristor, and and $\frac{d\Phi}{dq} = M(q)$ is the memristance of the memristor. Note that both equation \ref{fracmem} and equation \ref{rayleighmem} describe the Euler-Lagrange term of a dissipative element which is a function of the charge $q$, they are just derived using different techniques (one from the variation of a fractional action, and the other from the direct use of a Rayleigh dissipation function). By equating the final dissipation terms in the resulting E-L equations, we obtain:

\begin{equation}
    M(q)i(t) = \left( \frac{df}{dq} \right)^{2} i(t)
\end{equation}

And we see that the the nonlinear function $f(q)$ can be expressed in terms of the memristance $M(q)$ as:

\begin{equation}\label{memristance}
    \left( \frac{df(q)}{dq} \right)^{2} = M(q)
\end{equation}
